Extending Kubernetes Networking to make use of Segment Routing over IPv6 (SRv6)

Kubernetes is the leading platform for orchestrating containerized applications. In this paper, we extend Kubernetes networking to make use of SRv6, a feature-rich overlay networking mechanism. Integration with SRv6 can be very beneficial when Kubernetes is used in large-scale and distributed multi-datacenter scenarios. We have focused on the Calico CNI plugin, one of the most used Kubernetes networking plugins. In particular, we consider Calico-VPP, a version of the Calico plugin based on the VPP (Vector Packet Processing) data plane, which provides support for SRv6 operations with very high performance. The proposed SRv6 overlay networking solution for Kubernetes offers several advantages compared to a traditional overlay (e.g. IP in IP), in particular the possibility to use Traffic Engineering for the overlay tunnels. In the paper, we provide the architecture and the detailed design of the SRv6 based overlay and describe our open source implementation. We consider the research and technological question on how to extend Kubernetes networking to support large-scale and distributed multi-datacenter scenarios, which is an important goal for Cloud and Network providers. In this respect, we compare two different solutions for the control plane architecture of the SRv6 capable Kubernetes networking plugin, one based on the BGP routing protocol and another one based on extending the Kubernetes control plane. Finally, we report a performance evaluation of the data plane of the proposed SRv6 overlay networking, showing that it has comparable performance to existing overlay solutions (e.g. IP in IP), while offering a richer set of features.

==> nchapters/chapter1.tex <==
\chapter{State of Art}

\input{nchapters/kubernetes}
\input{nchapters/srv6}
\input{nchapters/vpp}
\input{sec/3-calico-vpp}

==> nchapters/chapter2.tex <==
\chapter{Overlay networking in Calico VPP}
\input{sec/4-ip-in-ip-calico}
\input{sec/5-srv6-overlay-calico-vpp}

==> nchapters/chapter3.tex <==
\chapter{Testbed and experiments}
\input{sec/7-results}


==> nchapters/chapter4.tex <==
\chapter{Kubernetes networking infrastructure testing platform}
\label{chap:kites}

As mentioned in the previous sections, networking in Kubernetes is one of the most critical as well as fundamental points.
Choosing the right network plugin is therefore a fundamental step to ensure good network performance within a Kubernetes cluster.
However, the evaluation of this performance could be a boring problem again. To solve these difficulties, we decided to design and develop a testing tool called \acrshort{KITESLabel} \cite{kites} (Kubernetes networking Infrastructure TESting platform)
\section{KITES (Kubernetes networking Infrastructure TESting platform)}
\label{sec:kitesintro}
The KITES platform is a tool capable of automatically evaluating the performance of the kubernetes infrastructure performance in an automatic way. Specifically, Kites aims to evaluate the performance of the cluster deployed and configured with a specific CNI.
Currently the supported CNI are
\begin{itemize}
    \item Calico with IPinIP
    \item Calico with \acrshort{VXLANLabel}
    \item Weave Net
    \item Flannel
\end{itemize}
KITES was developed to be used also in conjunction of an other testing platform called Kubernetes Playground \cite{k8s-playground} an automated, open-source, provisioner and configurator of Kubernetes environments designed to perform performance experiments against Kubernetes network plugins
\section{KITES: Architecture and workflow}
Kites consists of a series of bash scripts that allow to perform customized and automated assessments of the CNI deployed in a Kubernetes cluster. In particular, Kites was designed to be used in an already configured Kubernetes cluster composed of a variable number of worker nodes.
Kites must be placed and run on one of the cluster master nodes, in the default configuration it will perform a full performance analysis of the cluster, focusing on TCP and UDP traffic and a comprehensive analysis of the CPU utilization of the nodes directly involved in the ongoing experiment.
Moreover, to make Kites as flexible as possible, we have introduced a few parameters that allow a good level of customization of the tests that the user wants to perform:

\begin{itemize}
    \item Selection of the CNI deployed in the current cluster. This is a mandatory parameter that allows you to follow during the tests some specific flows that are closely related to the CNI.
    \item The number of worker nodes to test on.
    \item The type of test: UDP or TCP or both.
    \item The type of communication between pods: Pod to Pod on different nodes, Pod to Pod on the same node or same Pod.
    \item Enabling or disabling CPU monitoring.
\end{itemize}

Furthermore, as regards tests with UDP traffic we have provided KITES with the following options:

\begin{itemize}
    \item The size of the UDP packets. In particular, it is possible to specify multiple values separated by commas that allow the execution of the test for each size.
    \item The number of runs to be executed for each test.
    \item The amount of traffic load. It is possible to indicate the minimum and maximum number, with a customizable increment, of the number of packets per second (pps) to be analyzed.
\end{itemize}

We now describe the steps that Kites performs during the tests:
\begin{itemize}
    \item Clean up the environment, especially by clearing the data output folders from any previous experiments
    \item Create a Kubernetes namespace where the experiment pods and services will reside.
    \item Spawning the Pods that will take part in the tests. We use a DaemonSet to be able to spawn a Pod on each cluster node.
    \item Kites, after spawning the pods, collects all the necessary information about the resources created, such as: name, IP addresses and MAC address of each pod and creates a mapping with the node where the pod is located.
    \item If the UDP evaluation is enabled, Kites will create the ad hoc packet leveraging Trafgen \cite{trafgen}.
    \item At this point, everything is ready for testing. During this test, if enabled, Kites will start monitoring the CPU on each cluster node. It will then begin the execution by dividing it into two general groups:
    \begin{itemize}
        \item TCP traffic: test for the two types of communication: Pod to Pod and Pod to Node
        \item UDP traffic: test for the two types of communication: Pod to Pod and Pod to Node, moreover it performs a test for each traffic load and packet size defined at the beginning of the test.
    \end{itemize}
\end{itemize}

\section{Performance Indicators}
\label{sec:kitesperformanceindicator}
The current version of Kites is capable of evaluating two performance indicators: throughput and CPU utilization
\subsection{Throughput}
When it comes to throughput, Kites uses different tools and evaluation methods for TCP and UDP traffic. As far as TCP traffic is concerned, we have chosen iPerf \cite{iperf3}, which allows us to evaluate the maximum achievable throughput. Performing a measurement with iPerf assumes that there is one Pod server listening while the other Pod will behave as a client by sending a request to the server node. 
Although iPerf allows evaluations for UDP traffic, in this project it was decided to entrust the study to two different tools. The reason is that: in an attempt to generate high traffic rates, iPerf causes an extremely high processing load as found in the test results of paragraph \ref{sec:experiments}.
Specifically, we have opted for the adoption of the Netsniff \cite{netsniff} and Trafgen \cite{trafgen} tools, which both guarantee a zero-copy mechanism, in which upon receiving or transmitting a packet, the kernel does not need to copy it from the kernel from space to user space or vice versa.
Trafgen is a network traffic generator that allows ad-hoc customization of traffic, thanks also to a very powerful configuration language. In fact, this language supports a series of very useful features for the creation of packets, such as an integrated support for checksum of IP, UDP and TCP, a sort of constant expression evaluator, for example through bit shifting etc. Furthermore, Trafgen can also be used in fuzz testing contexts, that is, by configuring packages through random or following generators of particular expressions.
As described in \cite{trafgen}, by default, Trafgen starts as many processes as available CPUs,
pins each of them to their respective CPU and sets up the ring buffer each in their own process space after having compiled a list of packets to transmit. Thus, this is likely the fastest one can get out of the box in terms of transmission performance from user space, without having to load unsupported or non-mainline third-party kernel modules.
As mentioned above Trafgen, allows the creation of customized traffic using a powerful and simple configuration syntax, as reported in the example below:
\begin{lstlisting}[label=lst:trafgen, caption=Example of Trafgen packet definition,basicstyle=\ttfamily\large]
{
    /* -- Ethernet Header -- */
    ${MAC_ADDR_DST},
    ${MAC_ADDR_SRC},
    0x08, 0x00,
    /* -- IPv4 Header -- */
    0b01000101, 0,
    const16($IP_LEN),
    const16(2),
    0b01000000, 0,
    64,
    17,
    csumip(14, 33),
    /* -- UDP Header -- */
    ${IP_ADDR_SRC},
    ${IP_ADDR_DST},
    const16(9),
    const16(6666),
    const16($UDP_LEN),
    const16(0),
    /* -- Payload -- */
    fill('B', $PAYLOAD),
}
\end{lstlisting}
Netsniff, on the other hand, is a network packet analyzer capable of capturing or replicating pcap files. Netsniff supports a zero-copy facility achieved by using both Linux's RX\_RING and TX\_RING interfaces. This avoids the overhead of copying and system calls between the kernel and user address space.
\subsection{CPU usage}

Kites allows you to evaluate the average consumption used for each configuration of the measurements performed. 
The CPUs assigned to each node in the cluster, including the master node, were taken into consideration. The detection of the CPU in use is started at the beginning of each measurement performed. For example, before the start of communication from Pod 1, inside Node 1, and Pod 2, inside Node2, the measurement is started for the entire duration of the communication, which will therefore have as "tag" of TEST\_TYPE: k8s-worker-1TOk8s-worker-2. Therefore, these measurements are collected within machine readable files, marked by the type of communication: "samepod", "samenode" or "diffnode" with respective guest machines involved in communication.

Kites basically launches the well-known linux command top \cite{top} from within these machines. This command offers a series of information in realtime about the status of the machine, such as uptime, users connections, processes running, dormant, active, CPU status and memory usage

\section{Comparison with the state of the art}
\label{sec:kitescomparisonstateart}
As described in previous sections, I used kbn \cite{k8s-bench-suite} to evaluate the performance indicator of my work related to SRv6 in Calico VPP, which was the best solution at the time. However, we found that it was not designed to fit all of our use cases. For example, the first issues involved the lack of support for IPv6. Therefore, as described in \ref{sec:experiments} I had to modify the knb source code to support the IPv6 traffic tests, which are needed especially with SRv6. 


\begin{table}[ht]
\centering
\begin{tabularx}{1\textwidth}{|c|X|X|X|}
\toprule
Tool Name & Throughput & CPU & RAM \\ \midrule
knb & Yes & Yes & Yes \\
Kites & Yes & Yes & No \\ \bottomrule
\end{tabularx}
\caption{Comparison of the supported performance indicator}
\label{tab:kites-indicator-comparison}
\end{table}
Table \ref{tab:kites-indicator-comparison} provides a brief summary of the comparison with knb regarding the performance indicator. As it is easy to see, currently unlike knb, Kites does not have support for evaluating RAM consumption.

Table \ref{tab:comparison-kits-communication} provides a brief summary of the comparison with knb regarding the type of communication that can be tested. We can see that knb supports Pod to Service communication which is not supported by Kites yet and Kites supports Node to Pod communication which knb does not support.

\begin{table}[ht]
\centering
\begin{tabularx}{1\textwidth}{|c|X|X|X|}
\toprule
 & \multicolumn{1}{l}{Pod to Pod} & \multicolumn{1}{l}{Pod to Service} & \multicolumn{1}{l}{Node to  pod} \\ \midrule
knb & Yes & Yes & No \\
Kites & Yes & No & Yes \\ \bottomrule
\end{tabularx}
\caption{Configuration for performance experiments}
\label{tab:comparison-kits-communication}
\end{table}


==> nchapters/kubernetes.tex <==
\section{Kubernetes}
\label{sec:kubernetes}

Kubernetes is a portable, extensible, open source platform for managing containerized workloads and services, that facilitates both declarative configuration and automation \cite{kubernetesio}. Kubernetes facilitated the transition from "virtualized deployment era" to "container deployment era", providing a framework to run distributed systems resiliently.
In order to deploy a Kubernetes instance we need a cluster that is composed of a set of nodes that host the containerized applications. In general the nodes can be a physical machine or a virtual machine, for example deployed on top of a \acrshort{IaaSLabel} platform like OpenStack.
In addition, a node within the cluster can perform two functions as a master or as a worker, every cluster has at least one worker node.
\subsection{Kubernets basic components}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{fig/tesi/overall-kubernetes-cluster-components.pdf}
    \caption{View of a Kubernetes cluster main components}
    \label{fig:overall-kubernetes-cluster-components}
\end{figure}

As shown in fig \ref{fig:overall-kubernetes-cluster-components} we can distinguish for all the components of the cluster, the components of the Control Plan and the components of the node.
Let's now take a closer look at the components of these two subsets. 
The Control plane components make global cluster decisions, including scheduling, as well as detect and respond to cluster events, such as when starting a new pod the image version is not available. As described in \cite{kubernetesio-components} the components of this group can be run on any machine in the cluster, but in general it is best practice to start all control plane components on a machine that does not run user containers.

\subsubsection{Kube-apiserver}

The \acrshort{APILabel} server is a component of the Kubernetes control plane that exposes the Kubernetes API \cite{kubernetesio-components}. The API server is the front end for the Kubernetes control plane. The base implementation is kube-apiserver \cite{kube-apiserver}, which can be further extended through dedicated plugins.

\subsubsection{Etcd}

etcd is a consistent distributed key-value store, mainly used as a separate coordination service, in distributed systems. It is designed to hold small amounts of data that can fit entirely in memory \cite{etcd}. Etcd in the Kubernetes cluster is used as a backing store for all cluster data.

\subsubsection{Kube-scheduler}
Kube-scheduler is the component that watches for newly created Pods with no assigned node, and selects a node for them to run on \cite{kubernetesio-components}.  As described in \cite{kubernetesio-components} there are several factors that kube-scheduler can take into account for scheduling decisions: individual and collective resource requirements, hardware/software/policy constraints, affinity and anti-affinity specifications, data locality, inter-workload interference, and deadlines.

\subsubsection{Kube-controller-manager}

Kube-controller-manager is the component that handles all the kubernetes controller \cite{kubernetesio-controller} processes. In particular as described in \cite{kubernetesio-controller}, controllers are control loops that watch the state of your cluster, then make or request changes where needed. Example of controllers are:
\begin{itemize}
    \item Node controller, which has the task of monitoring the status of the nodes
    \item Job controller, which has the task of monitoring and managing the life cycle of Job objects
    \item Service Account controller: which has the task of creating the default accounts, when a new namespace \cite{kubernetesio-namespace} is created 
\end{itemize}


\subsubsection{Cloud-controller-manager}

The cloud-controller-manager only runs controllers that are specific to the cloud provider where the cluster is hosted. Specifically, it is designed to be fully integrated with public clouds, such as AWS or Azure, or even on an Openstack infrastructure, leveraging the cloud provider's API to maximize compatibility and correct use of available resources. Clearly, if we run Kubernetes on our premises, the cluster does not have a cloud controller manager. 
Example of controllers are:
\begin{itemize}
    \item Node controller, responsible for monitoring the status of a node in the cloud.
    \item Route controller, responsible for configuring routes in the underlying cloud infrastructure.
    \item Service controller: responsible for creating and monitoring interactions between the kubernetes service and the cloud provider's load balancer, through which the service is exposed.
\end{itemize}

Node components run on each node, with the purpose of both keeping pods running and providing the Kubernetes runtime environment \cite{kubernetesio-components}.

\subsubsection{Kubelet}
It is the main agent that runs on each node in the cluster, which has the task to make sure that containers are running in a Pod. As described in \cite{kubernetesio-components}, Kubelet actions depend on a set of PodSecs provided through various mechanisms and ensure that the containers described in those PodSpecs are running and healthy.

\subsubsection{Kube-proxy}
As described in \cite{kubernetesio-kube-proxy}Kube-proxy is the Kubernetes network proxy that runs on each node of the cluster, implementing part of the Kubernetes service concept, such as load balancing between pods, applying iptable rules to the traffic, manipulating packets, etc.
Kube-proxy maintains network rules on nodes. These network rules allow network communication to your Pods from network sessions inside or outside of your cluster.
It uses the packet filtering layer of the operating system, if it exists and is available. Otherwise, kube-proxy itself forwards the traffic.\\


In order to better understand some terms used in this thesis, other kubernetes objects are presented below.

\subsubsection{Pod}
As described in \cite{kubernetesio-concepts-pods} the smallest instantiable unit within a Kubernetes cluster is the Pod. A Pod contains one or more containers and has a unique IP address within the cluster. 
The containers within it share the same resources and the same network namespace, through which they can then communicate freely via the localhost address.
Usually each Pod contains a single container, except in cases where it can be useful to merge strongly coupled containers that also need to share resources.

\subsubsection{Namespace}
To ensure the isolation of its components, Kubernetes supports a mechanism called namespace. These namespaces provide a complete logical network stack with their own routers, firewalls, network devices, etc. \cite{kubernetesio-namespace}. 
In this way, no component within one namespace can affect the operation of another in a different namespace. Resources in each namespace are "invisible" to those in another namespace. This also avoids disambiguation problems between services with the same name.

\subsubsection{DaemonSet}
The DaemonSet is the resource that ensures that all (or some depending on the criteria declared in his definition) Nodes run a copy of a Pod. 
Furthermore, if a new node is available, the daemonset tries to automatically add the pods that are part of its definition to the node. Clearly, if a node is removed from the cluster or the policies on the node are changed, those pods running on that node are deleted. In our case as we will see in the next chapter the Daemonset is used by CNIs. 

\subsubsection{Service}
Pods are temporary objects, which means they can be stopped at any time due to errors or other causes, such as scheduling policies applied when the load on the cluster changes. 
When a Pod is terminated, its IP address is also deallocated and therefore a different address will be assigned to any "replacement" Pod. Hence the need to have the Services. 
Specifically, these resources provide a stable IP address and also balance the traffic between the Pods they are connected to. This ensures stability and reliability of communication within the cluster.

\subsubsection{ConfigMap}
As defined in \cite{config-map} a ConfigMap is an API object used to store non-confidential data in key-value pairs. Pods can consume ConfigMaps as environment variables, command-line arguments, or as configuration files in a volume. A ConfigMap allows you to decouple environment-specific configuration from your container images, so that your applications are easily portable.


\input{sec/2-k8s-model-cnis}




==> nchapters/srv6.tex <==
\section{Segment Routing over IPv6 (SRv6)}
\label{sec:srv6stateart}

The evolution of IP networks is driven by very challenging requirements, such as: i) the integration of tens of billions devices and of tens of millions of services in the cloud; ii) the support of very high capacity and/or very low latency interconnections, which may need to be accompanied with high availability and adequate security/privacy. Non-withstanding these challenging requirements, network operators needs also to reduce the operational and capital expenditures associated with the provisioning of their services. The softwarization of the network is obviously one of the answers to these trends, helping to cut costs and to provision a more scalable network. As a fundamental complement to the network softwarization, we present the SRv6 network architecture. SRv6 offers great benefits to network operators, service providers and users for the support of advanced services with a simplification of the network architecture and operations compared to the existing solutions for IP transport backbones (e.g. \paper{MPLS}\thesis{\acrshort{MPLSLabel}}, SR-MPLS).
Segment Routing (\paper{SR}\thesis{\acrshort{SRLabel}})~\cite{rfc8402, filsfils2015segment} is based on the \textit{loose Source Routing} concept. With Segment Routing, a node can include an ordered list of instructions (known as \textit{segments} in the packet headers. The segments can represent topological instructions (e.g. way points, steering the forwarding of the packets along a path in the network), or service based instructions (indicating the operations to be performed on the packet by a given node). The Segment List, which represents the instructions to be applied to a packet, can also be referred to as \textit{SR Policy}. Two instances of the SR Architecture have been designed and implemented, the earlier one is SR over MPLS (SR-MPLS)~\cite{rfc8660}, while SR over IPv6 (SRv6)~\cite{rfc8754} is the most recent one, which will be the focus of this chapter. SR over MPLS reuses the MPLS forwarding engines of IP backbone routers, based on the MPLS labels. The semantic of the MPLS labels is changed to represent the segments and the control plane of MPLS needs to be updated. We refer again the reader to~\cite{ventre2019survey} for further details on SR-MPLS.
The most important advantage of the Segment Routing architecture (in its two flavors, SR-MPLS and SRv6) is its great scalability with respect to traditional connection oriented architectures for IP backbones (e.g. traditional MPLS). Let us consider a single Traffic Engineering connection which needs to be setup using traditional MPLS. Assume that the connection spans 10 hops from ingress to egress. In addition to the traffic classification rules in the ingress node, an entry in the connection table of 10 nodes needs to be setup. This means that state information for a single connection needs to be maintained by 10 nodes and that, if an \paper{SDN}\thesis{\acrshort{SDNLabel}} approach is used, the SDN controller needs to interact with 10 nodes to setup the connection. With Segment Routing, only the state in the ingress node for the traffic classification is needed and the SDN controller needs to interact only with one node. A large network needs to support hundreds of thousands of connections, therefore the 10x saving in the number of state information (entries in the forwarding tables of nodes) and in the number of controller-to-node interactions that can be achieved with segment routing (considering 10 hops per connections) is a significant advantage. We note that the average number of segments needed to enforce a Traffic Engineered path is in the order of only 2 or 3 segments, as the packets will flow on normal IP shortest paths between one segment and the next one.  A further fundamental advantage, considering the Traffic Engineering aspects, is that in the path between one segment and the next one, it is possible to exploit \acrshort{ECMPLabel} (Equal Cost MultiPath), with gives a lot of benefits in terms of load balancing in the network, differently from traditional MPLS TE.

\subsection{SRv6 data plane}

The SRv6 data plane relies on a new type of IPv6 Routing Extension Header, called Segment Routing Header (SRH), defined in \cite{rfc8754}. The SRH contains the Segment List (SR Policy) as an ordered list of IPv6 addresses: each IPv6 address in the list is a \textit{Segment IDentifier} (SID). A dedicated field, called \textit{Segments Left}, is used to maintain the pointer to the active SID in the Segment List. The format of the SRH is shown in Fig.~\ref{fig:sr-header}.

In the SRv6 data plane (see Fig.~\ref{fig:srv6-data plane}), we consider three categories of nodes: Source SR nodes, Transit nodes and SR Segment Endpoint nodes. The Source SR node can be a host originating an IPv6 packet, or an ingress router at the border of an \textit{SR domain} which encapsulates the received packet. The latter scenario is depicted in Fig.~\ref{fig:srv6-data plane}, in which the Source SR node is an edge router that encapsulates a packet (which can be IPv6, IPv4 or even a Layer 2 frame) into an outer IPv6 packet and inserts the SR Header (SRH) as a Routing Extension Header in the outer IPv6 header. The encapsulated packet is indicated as Payload in Fig.~\ref{fig:srv6-data plane}. In this example, the Segment List in the SRH is composed of S1, S2 and S3 which are stored in reverse order in the SRH. The Segment Left field is set to 2, so that the active segment is S1, represented in red in the figure. The Source SR node sets the first SID of the SR Policy (S1) into the IPv6 Destination Address of the packet.

An SR Segment Endpoint node receives packets whose IPv6 destination address is locally configured as a segment. The SR Segment Endpoint node inspects the SR header and identifies the next segment in the Segment List, modifies the IPv6 destination address of the outer IPv6 header so that the identified next segment is copied in the IPv6 destination address and forwards the packet on the basis of the IPv6 forwarding table. In Fig.~\ref{fig:srv6-data plane}, we can see that S1 is the first SR Endpoint node, it decrements the Segment Left fields to 1, making S2 the active segment, and sets S2 as IPv6 destination address.

A Transit node forwards the packet containing the SR header based on the (outer) IPv6 destination address. In Fig.~\ref{fig:srv6-data plane}, nodes N4, N5, N6 and N7 are Transit nodes, which perform a regular forwarding of the packet toward the IPv6 destination address.


\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/tesi/sr-header.png}
    \caption{Segment Routing Header}
    \label{fig:sr-header}
%    \vspace{-3ex}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{fig/tesi/srv6-example.pdf}
    \caption{SRv6 data plane operations}
    \label{fig:srv6-data plane}
    \vspace{-3ex}
\end{figure}
%https://docs.google.com/presentation/d/1HwODULKVCEkbC6QVhbrX6WqWyUlv_JQ3/edit?dls=true
% pdf generated by gslide, verificare se funziona save as
% printing on PDF creator 
% ??? settings, advanced settings, papersize postscript custom page setup
% ??? width 118 mm height 230 mm % print quality 1200 dpi
% ??? true type download as softfonts
% ??? in powerpoint settings "High quality" from the slides print setting

\subsection{SRv6 Network Programming Model}

The SRv6 Network Programming model is defined in \cite{id-srv6-network-prog}. It consists of combining functions (\textit{SRv6 behaviors}) that can reside in different nodes to achieve \textit{a networking objective that goes beyond mere packet routing}. The Network Programming model offers the possibility to implement virtually any service by combining the basic behaviors in a \textit{network program} that is embedded in the packet header. 

The SRv6 Network programming model relies on the SRv6 data plane described in the previous subsection and provides a catalogue of behaviors that can be executed in SR source nodes (\textit{SR policy headend} behaviors) and in SR endpoint nodes (\textit{endpoint} behaviors). An SRv6 \textit{endpoint} behavior, also known as a behavior associated with a SID, represents a function to be executed on packets at a specific location in the network. Examples of behaviors described in \cite{id-srv6-network-prog} are the simple routing towards the next segment (\textit{End} behavior), the forwarding towards a specific next-hop (\textit{End.X} behavior), the decapsulation of a packet and the lookup into a specific IPv6 routing table (\textit{End.DT6} behavior, used to support Layer 3 \paper{VPN}\thesis{\acrshort{VPNLabel}} services). We refer the reader to \cite{ventre2019survey} for a deeper discussion on the SRv6 programming models. Several other behaviors are described in \cite{id-srv6-network-prog} (see also the table II of Section II.C in \cite{ventre2019survey}). It's worth noting that the behaviors described in \cite{id-srv6-network-prog} are not meant to be an exhaustive list, any advanced network function (e.g., firewall, NAT) that needs to be executed in a packet can be associated to a SID/instruction and included in a Network Program carried in a packet header. 

\subsection{SRv6 control plane}

Control Plane operations are needed to properly configure the SRv6 data plane. The fundamental operations are: i) the configuration of traffic classification and SR policies to be applied packets in the SR source nodes; ii) the association between Segment IDentifiers (SIDs) and instructions to be performed in a node (also known as SRv6 \textit{behaviors}). The plain intra-domain routing protocols (e.g. \paper{OSPF}\thesis{\acrshort{OSPFLabel}} and ISIS) are used to distribute the routing information for the reachability of nodes, which are also used by SRv6 basic topological instructions (way points). OSPF and ISIS are also being extended to distribute SRv6 specific information like node capabilities and the association between SIDs and service instructions (SRv6 behaviors). The SRv6 Control Plane operations can rely on a centralized SR controller that takes decisions and instructs the SR source nodes and the SR endpoints according to the SDN principles. Usually the distributed routing protocols and the centralized SDN approach are used in combination, resulting in a hybrid solution.

==> nchapters/vpp.tex <==
\section{Vector Packet Processor (\acrshort{VPPLabel}) platform}
\label{sec:vppstateart}

 The VPP platform \cite{whatisvpp} is an extensible framework that provides out-of-the-box production quality switch/router functionality \cite{whatisvpp}.

The benefits of this implementation of VPP are its high performance, proven technology, its modularity and flexibility, and rich feature set.
It is a modular design. The framework allows anyone to "plug in" new graph nodes without the need to change core/kernel code. 


%https://docs.google.com/drawings/d/1qz4wKCwioilkr_7g9I3Hrpg7TGQZGGYqmhVOrcLxlxA/edit

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/tesi/vpp-net-stack.pdf}
    \caption{VPP Packet Processing Layer In Network Stack Overview}
    \label{fig:vpp_net_stack}
\end{figure}


As described in \cite{whatisvpp} the VPP packet processing pipeline is decomposed into a packet processing graph , following a modular approach that allows anyone to extend the graph developing a component that can be plugged as a new graph node. Making the framework easily extensible for specific purposes.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{fig/tesi/vpp-graph.pdf}
    \caption{VPP custom application packet processing graph}
    \label{fig:vpp_graph}
\end{figure}

In order to understand how the plugin works \cite{whatisvpp} explains that at runtime VPP creates a vector of packets from the RX rings, generally with a size of 256 packets.
At this point, the packet processing graph is applied to the entire/full packet vector, processing the entire vector of packets through a graph node before moving on to the next one. In particular, the first packet processed from each vector creates a cache that is used to treat the subsequent ones. Graph nodes are small and modular, and loosely coupled. This makes it easy to introduce new graph nodes and rewire existing graph nodes.
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{fig/tesi/vpp-func-scalar.pdf}
    \caption{Scalar packet processing functions}
    \label{fig:vpp-func-scalar}
\end{figure}
As explained at \cite{scalarvsvector} FD.io, VPP relies on a vector packet processor rather than scalar packet processing. This means that, unlike scalar packet processing, VPP processes the packet vector, mentioned earlier, all at once. Specifically, an interrupt handling function takes the vector of packets from a network interface and processes it through a set of functions, as described in the figure below.
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{fig/tesi/vpp-func-vector.pdf}
    \caption{VPP vector packet processing functions}
    \label{fig:vpp-func-vector}
\end{figure}
As a result, the vector processing approach, compared to the scalar processing, solves:
\begin{itemize}
    \item (1)  the I-cache thrashing problem by amortizing the cost of I-cache loads across multiple packets
    \item (2) The inefficiencies associated with the deep call stack by receiving vectors of up to 256 packets at a time from the Network Interface, and processes them using a directed graph of nodes. The graph scheduler invokes one node dispatch function at a time, restricting stack depth to a few stack frames.
\end{itemize}





==> sec/8-related-work.tex <==
\section{Related work}
\label{sec:related}

VPP in Kubernetes (Contiv/Deprecated)

\url{https://s3-docs.fd.io/vpp/22.02/usecases/contiv/index.html}

\url{https://github.com/contiv/vpp}

==> uchapters/abstract.tex <==
\chapter*{Abstract}
\lettrine{K}ubernetes is considered the de facto system for automating deployment, scaling, and management of containerized applications. The growing cloudification of technology stacks, particularly in the telecommunications field, has highlighted the need to manage a large number of workloads, as well as the growing need to be able to distribute applications in geographically distributed datacenters.\\
Since the network model in Kubernetes is designed to be as generic as possible based on software components called CNI (Container Networking Interface) plugins, this makes it difficult to introduce specific network features for a CNI plugin cleanly, without interrupting compatibility with other plugins.\\
Segment Routing over IPv6 (SRv6) is a networking architecture that can be used in IP backbones and in data centers, where operators can implement services like overlay networking, VPNs, traffic engineering, protection/restoration in a scalable and effective way. Integrating a feature-rich network overlay solution, such as SRv6 with Kubernetes, would be very beneficial for service providers to address the challenges identified above, but currently no Kubernetes network plugin supports SRv6. \\
The first objective of this thesis is indeed the design and development of the extension of a CNI plugin to allow the support of SRv6 in the Kubernetes networking model. This extension is not trivial since, to be successfully deployed in the real world, it needs to be smoothly integrated into an existing CNI plugin without breaking existing features or compatibility. \\
Another problem is that IPv6 is currently not fully mature in Kubernetes networking plugins, while we need IPv6 for transport (as we want to use SRv6) and in the workload networks (where we want to support both IPv4 and IPv6). \\
A second set of issues that this thesis wants to solve, concerns the control and configuration mechanisms to be used in Kubernetes when dealing with the new advanced networking features. In fact, such features require the dynamic control and coordination of a potentially large number of nodes which could also be distributed in a large geographical area across multiple datacenters. \\
This thesis work shows how to design and implement an extension of a networking plugin (Calico-VPP) and its overlay solution based on IP-in-IP tunneling, implementing a custom IP-in-SRv6 tunneling. \\
One of the main results of this work is to ensure that the basic configuration of a Kubernetes cluster and its interaction with the CNI plugin is not changed, therefore our proposed solution can be completely transparent to Kubernetes users. \\
The thesis demonstrates that is possible to add advanced networking features with no disruption of the current CNI interface. Regarding the issues related to the control mechanism to be used to deal with the advanced networking features, this thesis work analyzes and implements two approaches: one is based on the extension of the BGP routing protocol and the other one is based on Kubernetes control plane.\\
As a result, the solution based on the BGP extension has been merged into the mainstream of the Calico-VPP project, while the one based on the Kubernetes control plane is still under evaluation.\\
Finally during the research activity, I found the need to have a tool to perform automated performance tests on the Kubernetes network plugins considering different types of traffic flows. In particular I found it necessary to support IPv6 and to be able to use the traffic generators most suitable for the type of transport protocol in use. Considering these requirements, I have worked on a tool called Kites, which has also been released as an open source project. 


==> uchapters/acronyms.tex <==
\newacronym[longplural={Container Network Interface}]{CNILabel}{CNI}{Container Network Interface}
\newacronym[longplural={Kubernetes}]{K8sLabel}{K8s}{Kubernetes}
\newacronym[longplural={Segment Routing for IPv6}]{SRv6Label}{SRv6}{Segment Routing for IPv6}
\newacronym[longplural={Segment Routing}]{SRLabel}{SR}{Segment Routing}
\newacronym[longplural={Network Layer Reachability Information}]{NLRILabel}{NLRI}{Network Layer Reachability Information}
\newacronym[longplural={Admission Control Lists}]{ACLsLabel}{ACLs}{Admission Control Lists} 
\newacronym[longplural={Segment IDentifier}]{SIDLabel}{SID}{Segment IDentifier}
\newacronym[longplural={Segment Routing Header}]{SRHLabel}{SRH}{Segment Routing Header}
\newacronym[longplural={Binding SID}]{BSIDLabel}{BSID}{Binding SID}
\newacronym[longplural={Software Defined Networking}]{SDNLabel}{SDN}{Software Defined Networking} %
\newacronym[longplural={Subsequent Address Family Identifier}]{SAFILabel}{SAFI}{Subsequent Address Family Identifier} 
\newacronym[longplural={IP Address Management}]{IPAMLabel}{IPAM}{IP Address Management}
\newacronym[longplural={Traffic Engineering}]{TELabel}{TE}{Traffic Engineering}
\newacronym[longplural={Virtual Machines}]{VMsLabel}{VMs}{Virtual Machines}
\newacronym[longplural={Vector Packet Processing}]{VPPLabel}{VPP}{Vector Packet Processing}
\newacronym[longplural={Maximum Transfer Unit}]{MTULabel}{MTU}{Maximum Transfer Unit}
\newacronym[longplural={Kubernetes Network Benchmark}]{knbLabel}{knb}{Kubernetes Network Benchmark}
\newacronym[longplural={Equal Cost MultiPath}]{ECMPLabel}{ECMP}{Equal Cost MultiPath}
\newacronym[longplural={Kubernetes networking Infrastructure TESting platform}]{KITESLabel}{KITES}{Kubernetes networking Infrastructure TESting platform}
\newacronym[longplural={Virtual Extensible LAN}]{VXLANLabel}{VXLAN}{Virtual Extensible LAN}
\newacronym[longplural={Infrastructure-as-a-Service}]{IaaSLabel}{IaaS}{Infrastructure-as-a-Service}
\newacronym[longplural={Network Address Translation}]{NATLabel}{NAT}{Network Address Translation}
\newacronym[longplural={Kernel-based Virtual Machine}]{KVMLabel}{KVM}{Kernel-based Virtual Machine}
\newacronym[longplural={Intermediate System to Intermediate System}]{ISISLabel}{ISIS}{Intermediate System to Intermediate System}
\newacronym[longplural={Multiprotocol Label Switching}]{MPLSLabel}{MPLS}{Multiprotocol Label Switching}
\newacronym[longplural={Application programming interface}]{APILabel}{API}{Application programming interface}
\newacronym[longplural={Data Plane Development Kit}]{DPDKLabel}{DPDK}{Data Plane Development Kit}
\newacronym[longplural={Host Networking Service}]{HNSLabel}{HNS}{Host Networking Service}
\newacronym[longplural={Virtual Private Network}]{VPNLabel}{VPN}{Virtual Private Network}
\newacronym[longplural={Open Shortest Path First}]{OSPFLabel}{OSPF}{Open Shortest Path First}
\newacronym[longplural={ Extended Berkeley Packet Filter}]{eBPFLabel}{eBPF}{ Extended Berkeley Packet Filter}

==> uchapters/conclusions.tex <==
\chapter*{Conclusions}
\markboth{Conclusions}{}
\input{sec/9-conclusions}

==> uchapters/contributions.tex <==
\chapter*{Contributions}

==> uchapters/introduction.tex <==
\chapter*{Introduction}
\markboth{Introduction}{}
\input{sec/1-introduction}
